Obscuration properties of mid-IR selected AGN

The goal of this work is to study the obscuration properties of mid-infrared (mid-IR) selected AGN. For that purpose, we use {\it{WISE}} sources in the Stripe 82-XMM area to identify mid-IR AGN candidates, applying the Assef et al. criteria. Stripe 82 has optical photometry $\approx$\,2 times deeper than any single-epoch SDSS region. XMM-Newton observations cover $\sim$26\,deg$^2$. Applying the aforementioned criteria, 1946 IR AGN are selected. $\sim 78\%$ have SDSS detection, while 1/3 of them is detected in X-rays, at a flux limit of $\rm \sim 5 \times 10^{-15}\,erg\,s^{-1}\,cm^{-2}$. Our final sample consists of 507 IR AGN with X-ray detection and optical spectra. Applying a $\rm r-W2>6$ colour criterion, we find that the fraction of optically red AGN drops from 43\% for those sources with SDSS detection to $23\%$ for sources that also have X-ray detection. X-ray spectral fitting reveals 40 ($\sim8\%$) X-ray absorbed AGN ($\rm N_H>10^{22}~cm^{-2}$). Among the X-ray unabsorbed AGN, there are 70 red systems. To further investigate the absorption of these sources, we construct Spectral Energy Distributions (SEDs) for the total IR AGN sample. SED fitting reveals that $\sim20\%$ of the optically red sources have such colours because the galaxy emission is a primary component in the optical part of the SED, even though the AGN emission is not absorbed at these wavelengths. SED fitting also confirms that $12\%$ of the X-ray unabsorbed, IR AGN are optically obscured.

==> README <==
fontaxes - Additional font axes for LaTeX
=========================================

The fontaxes package adds several new font axes on top of LaTeX's New Font
Selection Scheme. In particular, it splits the shape axis into a primary and
a secondary shape axis, and it adds three new axes to deal with the different
figure versions offered by many professional fonts.

Usage
-----

To use this package, include

    \usepackage{fontaxes}

in the preamble of your LaTeX document. See the PDF documentation for details.

Installation
------------

1. Run `latex fontaxes.ins` to generate the LaTeX package.

2. Create the following directories in a local texmf tree:

   - doc/latex/fontaxes
   - tex/latex/fontaxes

3. Copy all necessary files into the texmf tree:

   - fontaxes.pdf and test-fontaxes.tex go to doc/latex/fontaxes
   - fontaxes.sty goes to tex/latex/fontaxes

4. Afterwards, you may need to regenerate the file database:

    texhash

License
-------

Copyright (c) 2007 by Andreas Buehmann  
Copyright (c) 2014 by Michael Ummels <michael.ummels@rwth-aachen.de>

This work may be distributed and modified under the terms and conditions of the
LaTeX Project Public License, version 1.3c or greater (your choice).
The latest version of this license is in
  http://www.latex-project.org/lppl.txt
and version 1.3 or later is part of all distributions of LaTeX
version 2005/12/01 or later.

This work has the LPPL maintenance status `maintained'.

The Current Maintainer of this work is Michael Ummels.

This work consists of the files fontaxes.dtx, fontaxes.ins and
the derived files fontaxes.sty, test-fontaxes.tex and fontaxes.pdf.

